Fault-Tolerant Multi-Modal Localization of Multi-Robots on Matrix Lie Groups

Consistent localization of cooperative multi-robot systems during navigation presents substantial challenges. This paper proposes a fault-tolerant, multi-modal localization framework for multi-robot systems on matrix Lie groups. We introduce novel stochastic operations to perform composition, differencing, inversion, averaging, and fusion of correlated and non-correlated estimates on Lie groups, enabling pseudo-pose construction for filter updates. The method integrates a combination of proprioceptive and exteroceptive measurements from inertial, velocity, and pose (pseudo-pose) sensors on each robot in an Extended Kalman Filter (EKF) framework. The prediction step is conducted on the Lie group $\mathbb{SE}_2(3) \times \mathbb{R}^3 \times \mathbb{R}^3$, where each robot's pose, velocity, and inertial measurement biases are propagated. The proposed framework uses body velocity, relative pose measurements from fiducial markers, and inter-robot communication to provide scalable EKF update across the network on the Lie group $\mathbb{SE}(3) \times \mathbb{R}^3$. A fault detection module is implemented, allowing the integration of only reliable pseudo-pose measurements from fiducial markers. We demonstrate the effectiveness of the method through experiments with a network of wheeled mobile robots equipped with inertial measurement units, wheel odometry, and ArUco markers. The comparison results highlight the proposed method's real-time performance, superior efficiency, reliability, and scalability in multi-robot localization, making it well-suited for large-scale robotic systems.

==> Old_Introduction.tex <==
\IEEEPARstart{M}{obile} robots, whether operating individually or as part of a team, are widely deployed in indoor environments  to perform a variety of tasks, such as logistics, inspection, delivery, and quality control~\cite{}. To achieve automation for advanced navigation tasks such as path planning and mapping, these robots require  efficient localization systems. A key aspect of localization is the type of sensors used, leading to the development of various solutions for the self-localization of WMRs that integrate both proprioceptive and exteroceptive sensors. In indoor settings, wheel odometry~\cite{chong1997accurate} and inertial odometry using Inertial Measurement Unit (IMU)~\cite{barshan1995inertial} or fusion of them offer  simple, self-contained, and cost-effective methods~\cite{borenstein1996gyrodometry,cho2011dead,wang2023enhanced}. However, these approaches may not provide sufficient precision, as both wheel odometry and inertial sensors are prone to cumulative errors~\cite{borenstein1996measurement,barshan1995inertial}.
As the result, periodic global position updates are necessary to maintain accuracy. In GPS-denied environments, global localization can be achieved using (i) static or mobile anchors; (ii) passive or active landmarks; or (iii) map matching techniques~\cite{}. 

%%%%%%%%%%%%%%%%%%
In a multi-robot system, providing global localization for all agents is often impractical or costly. As a result, leader-follower Localization  has emerged as a  robust and scalable solution~\cite{mariottini2005vision,sharma2008cooperative,mariottini2007leader,van2020board}. In this approach, a subset of robots, known as leaders, rely on known or highly accurate global localization information, which they share with other robots, called followers, to help them estimate their positions. The leaders function as mobile anchors, providing reference position using estimation-based techniques such Extended Kalman Filter (EKF)~\cite{gottfried1965extended} by fusing global measurements with the onboard proprioceptive sensors such as IMU and encoders. While the followers use the leaders' communicated position along with their own onboard sensor data to estimate their positions through relative measurements. Passive fiducial markers, such as ArUco and AprilTag, are widely used in robotic systems for localization due to their high reliability, simplicity, and cost-effectiveness~\cite{kalaitzakis2021fiducial}. These markers can serve both as a source of global localization data and  determining relative pose between robots.



Another key aspect of estimation-based localization is the filtering mechanism used to fuse noise-corrupted data from multiple sensors. As the field progresses, a deeper understanding of the connections between matrix Lie groups, uncertainty representation, and advanced filtering techniques will continue to play a critical role in the development of more accurate and reliable localization systems for robotic applications. The robust representation provided by Lie groups inherently respects the geometric properties of motion, ensuring that operations such as composition, inversion, and fusion are efficient and meaningful. Furthermore, Lie groups enable the smooth handling of nonlinearities, as opposed to other representations such as Euler angles and quaternions that may suffer from singularities, discontinuities, and non-uniqueness~\cite{kenwright2013quaternions}.  

Building on the foundational concepts of pose representation and sensor fusion for localization, the following sections review relevant works on self-localization and leader-follower localization using fiducial markers. Additionally, they explore techniques for estimation and configuration operations within the framework of matrix Lie groups.


\subsection{Related works}

\subsubsection{Localization using Fiducial Markers}
  In estimation-based localization algorithms that incorporate fiducial markers, data is often fused in a two-step process: proprioceptive sensors data is incorporated during the prediction phase of estimation, while pose estimates from the fiducial markers are used to update the system’s state. The specific combination of sensors used in this fusion process can vary depending on the application. For instance,~\cite{zheng2018visual} relied on encoders, while IMU were used in~\cite{alatise2017pose}. In some studies, a combination of IMU, wheel encoders, and LiDAR have been explored~\cite{li2023indoor,chen2022marked}. 
Moreover, marker-based Simultaneous Localization and Mapping (SLAM) has become a significant research area, with early developments in~\cite{lim2009real}.
%%%%%%%%%
More recently, advancements in marker-based technologies have expanded to multi-robot systems.
A leader-follower control system combined with localization through sensor data fusion is proposed in~\cite{joon2023leader,joon2023leader}. The leader robot is equipped with four distinct ArUco markers, and additional markers are placed in the environment as landmarks. The follower robot is fitted with a  rotating camera to detect the ArUco markers. Localization of both robots is achieved by fusing IMU, encoder, and ArUco marker data through two Extended Kalman Filters (EKFs) on the follower and one EKF on the leader. A similar approach is presented in~\cite{zhou2021multi} for multi-robot cooperative localization, utilizing real-time communication and a two-stage EKF that fuses IMU and encoder data with relative pose measurements obtained from the ArUco marker on the slave robot. In~\cite{li2018cooperative} a marker-based cooperative localization method  that mimics a caterpillar-like motion was introduced. The method combines absolute pose estimates from static environmental features with relative pose estimates derived from known mobile fiducial markers while the fusion process is framed as an on-line optimization problem that integrates two distinct objectives from different feature sources. A leader–follower consensus protocol for networks of multiple non-holonomic mobile robots with fixed communication
topology is proposed in~\cite{jaoura2022distributed} in which the non-holonomic mobile robots move on a
platform with different ArUco markers on their tops and an overhead camera determines the robots poses. In~\cite{yang2023two}, a two-stage seamless switching strategy for positioning a mobile robot relative to a fixed manipulator was proposed. In this method, an ArUco marker is attached to the mobile robot, and its position is estimated using relative ArUco measurements when available. If these measurements are not accessible, an Extended Kalman Filter (EKF) is employed to fuse data from ultrasonic sensors and an IMU. The authors in~\cite{opromolla2022monocular} address spacecraft pose determination to facilitate the capture of a passively cooperative space target equipped with retro-reflective and black-and-white fiducial markers using a chaser platform equipped with a robotic arm. Fiducial markers are also used in design of controllers for multi-robot systems. For instance,~\cite{oh2023leader} proposed a position-based Leader‑follower formation control using
 relative observation of an ArUco marker attached on the leader. Furthermore, in~\cite{jayarathne2019vision} an ArUco marker was placed on the follower and based on the relative measurements a control law was designed for cooperative object handling. In~\cite{shan2016probabilistic}  a Bayesian leader-follower trajectory estimation has been presented in which the
follower robot estimates the trajectory of the leader robot based on the noise-corrupted odometry information of both robots, and relative observations of fiducial
markers.


\subsubsection{Estimation on Matrix Lie Groups}

Localization of systems evolving on matrix Lie groups centers around characterizing random pose variables on matrix Lie groups and their associate Lie algebras. The use of differential homogeneous transforms to represent uncertainty on the matrix Lie group 
$\mathbb{SE}(3)$ has been explored in earlier works such as~\cite{paul1981robot},\cite{durrant1987consistent}, and\cite{su1992manipulation}. These studies laid the groundwork for handling uncertainty propagation in the context of rigid body motion, with an emphasis on matrix representations of spatial transformations. A more comprehensive framework for expressing and advancing uncertainty on matrix Lie groups is presented in~\cite{wang2006error} and~\cite{chirikjian2011stochastic}, which extended the methods to address stochastic uncertainty modeling in robotics. This approach is further generalized to deal with uncertainty on general manifolds by~\cite{hertzberg2013integrating}, who introduced techniques for incorporating various sources of uncertainty.

Recent work by Long \textit{et al.} demonstrated that the observed probability distributions on 
$\mathbb{SE}(n)$ are normal in the exponential coordinates~\cite{long2013banana}. This result provides important insights into the use of exponential maps for uncertainty propagation in localization. Building on these advancements, Barfoot \textit{et al.}\cite{barfoot2014associating} proposed a framework for capturing pose uncertainties in the Lie algebra and using the exponential map to propagate these uncertainties for discrete-time variables on the Lie group 
$\mathbb{SE}(n)$. Their work emphasized the importance of Lie algebra for efficient uncertainty modeling and the application of exponential maps for transforming uncertainties in pose estimation tasks. This method was then extended for continuous-time random variables on  $\mathbb{SE}(3)$~\cite{tang2019white,wong2020data}. Furthermore, Mangelson \textit{et al.} extended these results to enable composition, inversion, and relative pose operations on two correlated pose estimates, while accounting for uncertainties in the Lie algebra\cite{mangelson2020characterizing}. This approach has been critical in real-time localization systems, where maintaining consistency across pose estimates is essential for high-precision localization. These advancements have enabled the researchers to develop consistent and efficient estimation solutions, such as the Extended Kalman Filter (EKF) on Lie groups~\cite{brossard2018exploiting, heo2018consistent}, the Invariant EKF (IEKF)~\cite{bonnabel2007left, xu2022distributed}, the Unscented Kalman Filter (UKF) on Lie groups~\cite{sjoberg2021lie, bohn2012unscented} and preintegration methods~\cite{forster2016manifold}.
%%%%%%%%%%%%%%%%%%%%%%

Fusion of estimates is a critical operation in localization systems, particularly in scenarios where multiple estimates of a process are available from different data sources. Building on the concept of naive fusion in vector spaces, Drummond et al.\cite{drummond2003computing} explore an iterative approach for combining two pose estimates. Non-iterative naive fusion techniques for multiple poses in 
$\mathbb{SE}(3)$ are also introduced in\cite{wolfe2011bayesian} and~\cite{long2013banana}. Expanding upon these methods, Barfoot et al.~\cite{barfoot2014associating} propose an iterative fusion method on 
$\mathbb{SE}(3)$ that minimizes a quadratic cost function encapsulating the error between local estimates and the current best fused estimate, approximated using the Baker–Campbell–Hausdorff (BCH) formula. Notably, this method simplifies the weighting matrix in the cost function by excluding cross-correlations and considering only individual covariances. Building on the naive fusion strategy, Hwang \textit{et al.}\cite{hwang2022novel} propose a federated Iterative Extended Kalman Filter (IEKF) for localization, which fuses estimates from two sub-filters updated based on left- and right-invariant observations. Adopting a similar error formulation and iterative framework to that of Barfoot \textit{et al.}\cite{barfoot2014associating}, Li \textit{et al.}\cite{li2021joint} introduce a split CI approach on Lie groups, which can accommodate correlated pose estimates. Additionally, distributed IEKF solutions based on the CI have been proposed in~\cite{xu2023distributed} and~\cite{xu2022distributed}. To avoid the iterative optimization used in~\cite{barfoot2014associating} and~\cite{li2021joint}, Petersen \textit{et al.}\cite{petersen2022tracking2} present a simpler, non-iterative fusion solution that uses the relative pose between local estimates and a reference estimate to define the error terms. This approach was further expanded to handle correlated pose estimates in\cite{zarei2024consistent}.


\subsection{Contributions}
This paper advances a novel fault-tolerant, estimation-based localization method for multi-robot systems consisting of Wheeled Mobile Robots (WMRs). The proposed approach efficiently fuses IMU and encoder data with pose observations from both fixed and mobile fiducial markers, using an EKF on Lie groups. The robot configurations are represented within the proposed matrix Lie group $\mathcal{G}\coloneq\mathbb{SE}_2(3)\times\mathbb{R}^3\times\mathbb{R}^3$, which encompasses position, rotation, velocity, and IMU biases. The process model is based on the kinematics of the IMU, and the EKF update is performed using encoder body velocity readings in $\mathbb{R}^3$. When fiducial marker observations are available, the EKF update incorporates both the encoder body velocity and pose measurements from the fiducial markers, thus resulting in an observation manifold of $\mathcal{G}_{\mathcal{Z}}\coloneq\mathbb{SE}(3)\times\mathbb{R}^3$.
To effectively integrate the fiducial marker observations, this paper develops operations on matrix Lie groups for stochastic configurations. To fully leverage the information available within the network, we introduce two types of information exchange between robots: leader-follower and follower-follower. When fixed fiducial marker observations are available for a leader, the developed stochastic operations are employed to generate pseudo-pose measurements, updating the leader's configuration using encoder data and pseudo-pose measurements on the measurement manifold $\mathbb{SE}(3)\times\mathbb{R}^3$. In the leader-follower communication protocol, The follower robots use the communicated leader locations along with relative observations of the mobile markers attached to the leaders to generate their own associative pseudo-pose measurements and update their locations on the manifold $\mathbb{SE}(3)\times\mathbb{R}^3$. Finally, the updated configuration of a follower, along with relative pose measurements from a fiducial marker attached to this follower, can be communicated to another follower, allowing the construction of pseudo-pose measurements for updates under the follower-follower communication protocol on $\mathbb{SE}(3)\times\mathbb{R}^3$.



\begin{itemize}
     
\item[(i)] This paper proposes stochastic configuration operations on an arbitrary matrix Lie group to perform composition, differentiation, inversion, and fusion of multiple random configurations. These operations are defined in the context of uncertainty on the right, with the assumption that the configurations may be either correlated or uncorrelated. In contrast to previous approaches~\cite{}, this work introduces a batch framework for the composition and fusion of more than two stochastic configurations. Additionally, it extends the concept of configuration to encompass not only pose but also other dynamic variables, e.g., extended pose.

\item[(ii)] We propose a novel multi-robot localization method for a network of WMRs that utilizes two types of information exchange: leader-follower and follower-follower. To achieve this, we fix fiducial markers in the environment and place mobile fiducial markers on each robot. We then apply the EKF on the Lie group to fuse IMU and encoder velocity data with pose measurements from the fiducial markers, which are processed through a sensor fault detection module. To the best of our knowledge, this is the first localization method that combines matrix Lie group concepts and sensor fault detection to fuse inertial odometry, wheel odometry, and fiducial marker data, while scaling cooperative localization across every robot in the network.


\item[(iii)] We have proposed a matrix Lie group framework for the EKF prediction step on the manifold $\mathbb{SE}_2(3)\times\mathbb{R}^3\times\mathbb{R}^3$, enabling the integration of IMU data. The configuration of each robot is updated on the manifold $\mathbb{R}^3$
  using encoder body velocity data. When fiducial markers and communicated poses are available—whether from a leader to a follower or between followers—the update is performed on the manifold 
$\mathbb{SE}(3)\times\mathbb{R}^3$
 . This update combines encoder velocity data with pseudo-pose measurements, which are constructed using the developed concepts of stochastic configuration composition and inversion.

 \item[(iv)] For the first time, we propose using configuration fusion for a follower robot that communicates with multiple robots, whether leaders or followers, and has access to the relative pose measurements of fiducial markers from each. This enables the fusion of two estimated configurations of this follower robot, resulting in enhanced performance.

\item[(v)] We have extended the concept of sensor fault detection on Lie groups by representing the measurements on  manifold and comparing them with the estimated values using the Mahalanobis distance metric. This approach effectively filters out faulty observations of fiducial markers, ensuring robust estimation performance.


\end{itemize}



